LoRea: A Backscatter Architecture that Achieves a Long Communication Range

There is the long-standing assumption that radio communication in the range of hundreds of meters needs to consume mWs of power at the transmitting device. In this paper, we demonstrate that this is not necessarily the case for some devices equipped with backscatter radios. We present LoRea an architecture consisting of a tag, a reader and multiple carrier generators that overcomes the power, cost and range limitations of existing systems such as Computational Radio Frequency Identification~(CRFID). LoRea achieves this by: First, generating narrow-band backscatter transmissions that improve receiver sensitivity. Second, mitigating self-interference without the complex designs employed on RFID readers by keeping carrier signal and backscattered signal apart in frequency. Finally, decoupling carrier generation from the reader and using devices such as WiFi routers and sensor nodes as a source of the carrier signal. An off-the-shelf implementation of LoRea costs 70 USD, a drastic reduction in price considering commercial RFID readers cost 2000 USD. LoRea's range scales with the carrier strength, and proximity to the carrier source and achieves a maximum range of 3.4 kilometre when the tag is located at 1 meter distance from a 28 dBm carrier source while consuming 70 microwatts at the tag. When the tag is equidistant from the carrier source and the receiver, we can communicate upto 75 meter, a significant improvement over existing RFID readers.

==> design-tag.tex <==
% vim: textwidth=72 spell spelllang=en_us

\fakeparagraph{FSK} We also implement frequency shift keying on the
commodity MCU. We use the MSP430 FR5696, a low-power MCU from the
popular MSP430 family that has seen widespread adoption in the IoT
community.

In our implementation, a 0-bit is represented by a frequency $f_0$ and a
1-bit is represented by another frequency $f_1 = f_0 +
190~\mathrm{kHz}$; i.e., the two frequencies are spaced 190~kHz apart.
To unburden the reader from interference cancellation, the frequencies
are shifted by $f_\Delta$, thereby achieving the aforementioned mixing
property.
%
We use the MSP430's timer to generate a square wave with a frequency of
$f_\Delta+f_0$ to transmit a 0-bit and a frequency of $f_\Delta+f_1$ to
transmit a 1-bit. The timer's output is routed to a GPIO pin, which
in turn toggles the TX state of the connected antenna front-end.
Following the reasoning of §\ref{}, this allows the tag to modulate the
carrier using frequency shift keying. The reader can demodulate the
transmission at a channel frequency of $f_\mathrm{carrier} \pm
f_\Delta$.


==> introduction.tex <==
Backscatter  has attracted significant recent interest to
enable battery-free devices~\cite{ambientbackscatter} and to reduce communication 
costs on mobile devices~\cite{braidio}.  Backscatter modulates ambient 
radio signals by
reflecting or absorbing them, which consumes only
sub $\mu W$ of power~\cite{hmc190}.  
The ultra low power nature makes it possible 
to network battery-free
sensors operating in severe 
energy harvesting conditions~\cite{ambientbackscatter,zhang2014enabling}.
Despite these advantages, and a decade of research efforts~\cite{oldwisp,zhang2011moo}, 
embedded sensing applications using backscatter have been far and few owing
to the restrictions due to the readers.

CRFID platforms 
like WISP~\cite{oldwisp} and Moo~\cite{zhang2011moo} have
been  widely used to conceive novel backscatter
applications, like battery-free  
cameras~\cite{wispcam}, 
activity monitoring~\cite{batteryactivity}
or localisation~\cite{zhao2013battery}. 
CRFID platforms, while offer high degree of
configurability of  hardware and firmware,
are constrained due to the readers
used to query them.

RFID readers employed to query CRFID platforms
are designed to query passive RFID tags, which 
exchange only few bytes of 
identification data~( EPC Gen 2, a commonly used RFID protocol only   
allows 12 $bytes$ of identification data )
Restrictions on the  payload makes it 
difficult to support sensors which transmit large amounts
of data~\cite{6548159}. For example,  
Naderiparizi et al. implements a battery-free camera, 
as streaming large amounts of data is difficult, 
they buffer and slowly transfer the data to the RFID readers increasing the
latency between frame captures~\cite{wispcam}. RFID readers, thus, restricts applications
of CRFID platforms to only very low throughput sensing application.

RFID readers generate a strong carrier signal~(approx 1 $W$) to both query
and deliver energy to passive RFID tags. 
CRFID tags, consequently, couple together both the 
RF-based energy harvesting together with the
communication, even though this has been shown to be inefficient 
owing to asymmetric communication
and harvesting range~\cite{gummeson2010limits,sample2011photovoltaic,zhang2014enabling}.
The strong carrier also increases the cost and complexity of the reader due to 
the need to reduce strong self-interference~\cite{braidio}, making them prohibitively 
expensive for many applications~(approximately 2000 USD)~\cite{impinj}. RFID readers are
also restricted in communication range, and can only communicate
with CRFID tags upto few meters~\cite{zhang2014enabling}
restricting their use in real applications. 

In summary, the present CRFID platforms
are severely constrained due to the intricacies
of the RFID readers, and restricts
the possible  applications, and there is need to redesign
of the backscatter platforms and the readers.





\fakepar{Contributions}  To overcome the limitations of the present CRFID based
backscatter platforms and readers, we design \system.
\system is a low cost,
high range and high throughput
backscatter reader that overcomes 
limitations of the conventional RFID readers.
\system achieves high 
performance by taking advantage of a number of design choices: 
First, by taking advantage of cheap
off-the-shelf~(approx 5 USD) available radio 
transceivers which offer very high sensitivity, \system
achieves low cost and high range. 
Second, as opposed to traditional RFID communication,
\system separates the backscatter transmissions from the
carrier by shifting the weak backscattered signal away
from the carrier signal easing the need for complex 
techniques to reduce self-interference and 
helping to keep the cost of the reader low.
Finally, to improve performance,
lower power consumption, and keep
reduce self interference, \system decouples the carrier 
generation from the reader, making it possible to
use deployed infrastructure like smartphones and
sensor devices to provide the carrier.


In summary, we make the following contributions with
the design of  \system backscatter reader:

\begin{itemize}
\item \system reader costs~(approx 70 USD), while achieving range of $200+$ meters
 	  in line of sight, which is orders of magnitude higher than achieved using RFID readers,
 	  and 6 $\times$ higher than Passive WiFi~\cite{kellogg2016passive}, and 4 $\times$ higher than HitchHike~\cite{HitchHike}, the
	  two recent backscatter systems.

	  
\item \system by decoupling carrier generation from reader, enables deployed infrastructure 
	  of smartphones and sensor devices to generate carrier signal to query backscatter tags
	  improving the range and scalability of the system.
	  
\item \system allows commodity MCUs to generate baseband signals making it possible to network
	  billions of existing deployed devices using backscatter communication. 
	  
\end{itemize}



The paper proceeds as follows, in the Section XX, we discuss the related work, in Section YY, we 
provide background of existing backscatter readers and tags. In Section 4, we discuss the design
of the \system.  In Section 5, we evaluate the system under different test conditions. In Section 6,
we present use cases. Finally, we conclude the paper.















2


==> outdoor.tex <==







\begin{figure}[!tb]
\centering
\includegraphics[width=0.37\textwidth]{results/outdoorbercg.pdf}
\caption{\capt{Performance in  line of sight outdoors for different distances between backscatter tag and carrier generator.}  The vertical dashed lines indicate presence of  wall.
At the lowest bitrate
we can achieve a range of 29 meters while traversing 8 walls. }
\label{throughwall}
\end{figure}


\begin{figure}[!tb]
\centering
\includegraphics[width=0.37\textwidth]{results/outdoor_lowbitrate_tagreceiver.pdf}
\caption{\capt{Performance in  line of sight outdoors for distances between backscatter tag and  the receiver.} As the distance from the carrier generator
increases, the receiver needs to be positioned more closely to the backscatter tag.}
\label{outdoorbtagrcvr}
\end{figure}

\begin{figure}[!tb]
\centering
\includegraphics[width=0.37\textwidth]{results/highspeed_tagcarrier.pdf}
\caption{\capt{High bitrate  reader mode (Outdoors).} As distance between the backscatter tag and the carrier generator increase the bit errors increase. We see lower range and higher bit errors as compared to low bitrate mode of the reader.}
\label{outdoorhighber}
\end{figure}



==> passive.tex <==





==> readersrelated.tex <==
There have been some prior attempts to develop
low-cost backscatter readers. Braidio is a 
backscatter reader that can switch between
 active and passive
radios depending on the energy constraints of the
host device~\cite{braidio}.  Similar to our 
solution, Braidio can function as a low-cost and low-power
backscatter reader, but 
achieves a range of \SI{1.8}{\metre} at \SI{100}{kbps}.
As a comparison,  we can reach beyond \SI{600}{\metre} due to three primary 
reasons: First, Braidio uses passive receivers similar to the ones found
on RFID
tags resulting in a sensitivity
of approximately \SI{-60}{dBm}. By contrast, the receivers employed 
in our architecture are narrow-band radios 
with high sensitivity levels. Second, 
 we separate the weak backscattered signal from the strong carrier
 which improves the SNR of the backscattered transmissions. 
 Finally, we  enable bi-static operation of
the reader which helps further reduce self-interference.
Another notable attempt is from Nikitin~et~al, who design
a simple and low-cost reader~\cite{nikitin2013simple}
but achieve a range of only \SI{15}{cm}.



\fakepar{Self-interference mitigation}
There has been significant recent work 
to reduce self-interference and enable
full-duplex operations on radios~\cite{Jain:2011:PRF:2030613.2030647,Choi:2010:ASC:1859995.1859997,Bharadia:2014:FDM:2616448.2616482}.
These techniques, however, significantly increase the complexity, power consumption and cost of the reader.

Liu et al. present a design to reduce self-interference and enable
full-duplex operation on ambient backscatter devices~\cite{Liu:2014:EIF:2639108.2639136}. 
These designs achieve only few meters of range.\tv{plural (these). Do you refer to Liu only or also all the above?}
Recent backscatter systems leverage the spectral mixing property
of backscatter transmissions to 
shift backscatter transmissions away from the carrier to
reduce self-interference~\cite{kellogg2016passive,HitchHike,blebackscatter,passivesensortags,passivezigbee,zhang_enabling_2016}.
We build upon these recent designs to develop an efficient reader
for CRFID devices that achieves a high communication range at low cost.



Ma et al.~\cite{ma16loc} use non-linear elements
attached to the WISP platform to reduce self-interference
and achieve accurate 3D localization.
While Ma et al.~\cite{ma16loc} also reduce self-interference, 
we target a different problem: by shifting
the carrier we reduce self-interference to lower the cost of
the backscatter reader and enable higher communication ranges.


==> related.tex <==
This section begins with a summary of other efforts in designing low-power backscatter readers
followed by an overview of CRFID platforms, we next discuss briefly
self-interference mitigation and finally discuss recent backscatter systems.







%Furthermore, HitchHike, together with the replica occupies almost
%half of available 
%creates a replica image of  WiFi transmission
%~($\sim$ 20 $MHz$). Together with the replica image, HitchHike
%transmissions occupy half of the available~( $\sim$ 40 $MHz$) 
%spectrum at ISM bands which could further aggravate cross technology 
%interference.   







==> usecase.tex <==
\subsection{Campus wide backscatter}
\subsection{Battery free push button}
